Can Vision Language Models Learn from Visual Demonstrations of Ambiguous Spatial Reasoning?

Large vision-language models (VLMs) have become state-of-the-art for many computer vision tasks, with in-context learning (ICL) as a popular adaptation strategy for new ones. But can VLMs learn novel concepts purely from visual demonstrations, or are they limited to adapting to the output format of ICL examples? We propose a new benchmark we call Spatial Visual Ambiguity Tasks (SVAT) that challenges state-of-the-art VLMs to learn new visuospatial tasks in-context. We find that VLMs fail to do this zero-shot, and sometimes continue to fail after finetuning. However, adding simpler data to the training by curriculum learning leads to improved ICL performance.

==> tables/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{wraptable}{r}{0.38\textwidth}
\scriptsize
\caption{Ablation study}
\label{tab:ablation}
\begin{tabular}{@{}lcc@{}}
\toprule
Method          & MiniCPM        & VILA \\ \midrule
Best Curriculum & 75.1           & 63.8 \\
More Data       & 57.3 (-23.7\%)  & 50.7 \\
More Epochs     & 64.2 (-14.5\%) & 50.8 () \\
Mixed Data      & 73.5 (-2.1\%)  &      \\ \bottomrule
\end{tabular}
\end{wraptable}

==> tables/curriculum.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t!]
\centering
\small
\caption{VLMs' performance on the task family $\varphi = (\mathbb{I}_5, \mathbb{C}_{\text{hard}}, 3)$ after curriculum learning, together with each metric's relative improvements compared to the finetuned model. \todo{use fig.}}
\label{tab:curriculum-learning}
\begin{tabular}{@{}lccccc@{}}
\toprule
Curriculum                 & LLaVA-Next & VILA           & IDEFICS2       & InternVL2 & MiniCPM        \\ \midrule
$\mathcal{C}^{\mathbb{I}}$ & 48.5 (-7.3\%) & 50.9 (+0.6\%)  & 49.0 (+0.8\%)  & 53.1 (+4.3\%) & 64.6 (+4.0\%)  \\
$\mathcal{C}^{\mathbb{C}}$ & \textbf{62.5 (+19.5\%)} & 51.0 (+0.8\%) & 50.8 (+4.5\%) & \textbf{68.3 (+34.2\%)} & 63.1 (+1.6\%)  \\
$\mathcal{C}^{M}$          & 49.8 (-4.8\%)  & 55.2 (+9.1\%) & 51.9 (+6.8\%) & 53.3 (+4.7\%)  & \textbf{75.1 (+20.9\%)} \\
$\mathcal{C}^{\text{all}}$ & 57.7 (+10.3\%) & \textbf{63.8 (+26.1\%)} & \textbf{55.5 (+14.2\%)} & 59.7 (+17.3\%) & 73.4 (+18.2\%) \\ \bottomrule
\end{tabular}
\end{table}
